Learn molecular representations from large-scale unlabeled molecules for drug discovery

How to produce expressive molecular representations is a fundamental challenge in AI-driven drug discovery. Graph neural network (GNN) has emerged as a powerful technique for modeling molecular data. However, previous supervised approaches usually suffer from the scarcity of labeled data and have poor generalization capability. Here, we proposed a novel Molecular Pre-training Graph-based deep learning framework, named MPG, that leans molecular representations from large-scale unlabeled molecules. In MPG, we proposed a powerful MolGNet model and an effective self-supervised strategy for pre-training the model at both the node and graph-level. After pre-training on 11 million unlabeled molecules, we revealed that MolGNet can capture valuable chemistry insights to produce interpretable representation. The pre-trained MolGNet can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of drug discovery tasks, including molecular properties prediction, drug-drug interaction, and drug-target interaction, involving 13 benchmark datasets. Our work demonstrates that MPG is promising to become a novel approach in the drug discovery pipeline.

==> table1.tex <==

\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{LightGreen}{rgb}{0.88,1,0.88}
\definecolor{LightRed}{rgb}{1,0.88,0.88}
\definecolor{LightGray}{gray}{0.8}

\begin{table}[]

    \centering
    \caption{The performance comparison. The numbers in brackets are the standard deviation. The methods in green are pre-trained methods.}
 \resizebox{0.9\textwidth}{!}{
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{ccccccc}
\hline
\multicolumn{7}{c}{Classification (AUC-ROC)} \\
\hline
Dataset & {BBBP} & {SIDER} & {ClinTox} & {BACE} & {Tox21} & {ToxCast} \\
\# Molecules & {2039} & {1427} & {1478} & {1513} & {7831} & {8575} \\
\hline
TF\_Robust \cite{ramsundar2015massively} & $0.860_{(0.087)}$ & $0.607_{(0.033)}$ & $0.765_{(0.085)}$ & $0.824_{(0.022)}$ & {$0.698_{(0.012)}$} & $0.585_{(0.031)}$ \\
GraphConv \cite{kipf2016semi}& $0.877_{(0.036)}$ & $0.593_{(0.035)}$ & $0.845_{(0.051)}$ & $0.854_{(0.011)}$ & {$0.772_{(0.041)}$} & $0.650_{(0.025)}$ \\
Weave  \cite{kearnes2016molecular}& $0.837_{(0.065)}$ & $0.543_{(0.034)}$ & $0.823_{(0.023)}$ & $0.791_{(0.008)}$ & {$0.741_{(0.044)}$} & $0.678_{(0.024)}$ \\
SchNet \cite{schutt2017schnet}& $0.847_{(0.024)}$ & $0.545_{(0.038)}$ & $0.717_{(0.042)}$ & $0.750_{(0.033)}$ & {$0.767_{(0.025)}$} & $0.679_{(0.021)}$ \\
MPNN  \cite{gilmer2017neural}& $0.913_{(0.041)}$ & $0.595_{(0.030)}$ & $0.879_{(0.054)}$ & $0.815_{(0.044)}$ & {$0.808_{(0.024)}$} & $0.691_{(0.013)}$ \\
DMPNN \cite{yang2019analyzing}&  $0.919_{(0.030)}$ &  $0.632_{(0.023)}$ & $0.897_{(0.040)}$ & $0.852_{(0.053)}$ & { $0.826_{(0.023)}$} &  $0.718_{(0.011)}$ \\
MGCN  \cite{lu2019molecular}& $0.850_{(0.064)}$ & $0.552_{(0.018)}$ & $0.634_{(0.042)}$ & $0.734_{(0.030)}$ & {$0.707_{(0.016)}$} & $0.663_{(0.009)}$ \\
AttentiveFP \cite{xiong2019pushing}& $0.908_{(0.050)}$ & $0.605_{(0.060)}$ &  $0.933_{(0.020)}$ &  $0.863_{(0.015)}$ & {$0.807_{(0.020)}$} & $0.579_{(0.001)}$ \\
\hline
\cellcolor{LightGreen}N-GRAM \cite{liu2019n}& $0.912_{(0.013)}$ & $0.632_{(0.005)}$ & $0.855_{(0.037)}$ &  $0.876_{(0.035)}$ & {$0.769_{(0.027)}$} & -\footnotemark \\
\cellcolor{LightGreen}HU. et.al\cite{hu2019strategies} & $0.915_{(0.040)}$ & $0.614_{(0.006)}$ & $0.762_{(0.058)}$ & $0.851_{(0.027)}$ & {$0.811_{(0.015)}$} & $0.714_{(0.019)}$ \\

%\cellcolor{LightGreen}${GROVER}_{base}$ & $0.936_{(0.008)}$ & $0.656_{(0.06)}$ & $0.925_{(0.013)}$ & $0.878_{(0.016)}$ & {$0.819_{(0.020)}$} & $0.723_{(0.010)}$ \\
\cellcolor{LightGreen}${GROVER\cite{rong2020grover}}$ & 
${0.940}_{(0.019)}$ & 
${0.658}_{(0.023)}$ & 
${0.944}_{(0.021)}$ & 
${0.894}_{(0.028)}$ & {${0.831}_{(0.025)}$} & ${0.737}_{(0.010)}$ \\
\hline
\cellcolor{LightCyan}${MPG}$ & 
\cellcolor{LightCyan}$---_{(---)}$ & 
\cellcolor{LightCyan}$\bm{0.658}_{(0.012)}$ & 
\cellcolor{LightCyan}$\bm{0.963}_{(0.028)}$ &
\cellcolor{LightCyan}$\bm{0.920}_{(0.013)}$ & 
{\cellcolor{LightCyan}$\bm{0.837}_{(0.019)}$} & \cellcolor{LightCyan}$\bm{0.748}_{(0.005)}$ \\

\hline


\hline
\hline
\multicolumn{7}{c}{Regression (RMSE)} \\
\hline
Dataset & {FreeSolv} & {ESOL} & {Lipo}  \\
\# Molecules & {642} & {1128} & {4200} &  \\
\cline{1-4}TF\_Robust \cite{ramsundar2015massively} & $4.122 _{(0.085)}$ & $1.722 _{(0.038)}$ & $0.909 _{(0.060)}$ &  \\
GraphConv \cite{kipf2016semi}& $2.900_{(0.135)}$ & $1.068_{(0.050)}$ & $0.712_{(0.049)}$ &  \\
Weave  \cite{kearnes2016molecular}& $2.398_{(0.250)}$ & $1.158_{(0.055)}$ & $0.813_{(0.042)}$ &  \\
SchNet \cite{schutt2017schnet}& $3.215_{(0.755)}$ & $1.045_{(0.064)}$ & $0.909_{(0.098)}$ &   \\
MPNN  \cite{gilmer2017neural}& $2.185_{(0.952)}$ & $1.167_{(0.430)}$ & $0.672_{(0.051)}$ &  \\
DMPNN \cite{yang2019analyzing}& $2.177_{(0.914)}$ & $0.980_{(0.258)}$ & $0.653_{(0.046)}$ & \\
MGCN  \cite{lu2019molecular}& $3.349_{(0.097)}$ & $1.266_{(0.147)}$ & $1.113_{(0.041)}$ &  \\
AttentiveFP \cite{xiong2019pushing}&  $2.030_{(0.420)}$ &  $0.853_{(0.060)}$ &  $0.650_{(0.030)}$ &  \\
 \cline{1-4}\cellcolor{LightGreen}N-GRAM \cite{liu2019n}& $2.512_{(0.190)}$ & $1.100_{(0.160)}$ & $0.876_{(0.033)}$ & \\
%\cellcolor{LightGreen}$GROVER_{\text{base}}$ & $1.592_{(0.072)}$ & $0.888_{(0.116)}$ & $0.563_{(0.030)}$ & $\bm{72.5}_{(5.9)}$ & $0.0172_{(0.002)}$ &  \\
\cellcolor{LightGreen}${GROVER\cite{rong2020grover}}$ &  $\bm{1.544}_{(0.397)}$ & $\bm{0.831}_{(0.120)}$ &  $\bm{0.560}_{(0.035)}$ &  \\
% \hline
\cline{1-4}\cellcolor{LightCyan}${MPG}$ & 
\cellcolor{LightCyan} $\bm{1.269}_{(0.192)}$ &
\cellcolor{LightCyan} $\bm{0.802}_{(0.023)}$ & 
\cellcolor{LightCyan} ${0.576}_{(0.029)}$ &
 \\
\hline
\end{tabular}%
}
\vspace{-2ex}
\label{tab:performance_res}
\end{table}
